Interpretable Representation Learning of Cardiac MRI via Attribute Regularization

Interpretability is essential in medical imaging to ensure that clinicians can comprehend and trust artificial intelligence models. Several approaches have been recently considered to encode attributes in the latent space to enhance its interpretability. Notably, attribute regularization aims to encode a set of attributes along the dimensions of a latent representation. However, this approach is based on Variational AutoEncoder and suffers from blurry reconstruction. In this paper, we propose an Attributed-regularized Soft Introspective Variational Autoencoder that combines attribute regularization of the latent space within the framework of an adversarially trained variational autoencoder. We demonstrate on short-axis cardiac Magnetic Resonance images of the UK Biobank the ability of the proposed method to address blurry reconstruction issues of variational autoencoder methods while preserving the latent space interpretability.

==> TABLES/attributes.tex <==
\begin{tabular}{m{0.4\textwidth} p{0.25\textwidth}>{\centering\arraybackslash}p{0.2\textwidth}}
        \toprule
	 \multicolumn{1}{c}{\textbf{Attribute}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Range}} \\
	\midrule
	  Left Ventricular EDV & LVEDV (mL) & 158.32 $\pm$ 38.23 \\ 
        Myocardial EDV & MyoEDV (mL) & 79.83 $\pm$ 20.90\\
        Right Ventricular EDV & RVEDV (mL) &148.12 $\pm$ 33.95 \\ 
        Left Ventricular ESV &  LVESV (mL) &   68.58 $\pm$ 21.92 \\
        Myocardial ESV & MyoESV (mL) & 79.83 $\pm$ 20.90\\
        Right Ventricular ESV & RVESV (mL) & 60.41 $\pm$ 19.17 \\     
	\bottomrule
\end{tabular}




==> TABLES/classification.tex <==
\resizebox{1\textwidth}{!}{
\begin{tabular}{lcccccc}
		\toprule
		
		Input & Method & AUROC & Accuracy & Precision & Recall & F1-Score \\ 
        \midrule
	
		LVEF & Regression & 0.57  & 0.57	&  0.57  & 0.58 &  0.57 \\
        Attributes & Regression &  0.65  & 0.65 & 0.67  & 0.58  &  0.62 \\		
        Images & ResNet-18 &    &  &   &  & \\

        Images + Attr. & Attri-VAE & 0.53  & 0.49 & 0.58 & 0.52 & 0.41 \\
        Images + Attr. & AR-SIVAE &  0.50  & 0.52 & 0.58  & 0.55  &  0.50 \\
        Images + Attr. & AR-SIVAE + MLP &  0.53  & 0.53 & 0.53  & 0.53  &  0.53 \\
    \midrule

    Mesh  & From \cite{Beetz:2023} & 0.77 & 0.69 & 0.70 & 0.68 & 0.70 \\
    
	\bottomrule       
\end{tabular}
}


